Reading Between the Frames: Multi-Modal Depression Detection in Videos from Non-Verbal Cues

Depression, a prominent contributor to global disability, affects a substantial portion of the population. Efforts to detect depression from social media texts have been prevalent, yet only a few works explored depression detection from user-generated video content. In this work, we address this research gap by proposing a simple and flexible multi-modal temporal model capable of discerning non-verbal depression cues from diverse modalities in noisy, real-world videos. We show that, for in-the-wild videos, using additional high-level non-verbal cues is crucial to achieving good performance, and we extracted and processed audio speech embeddings, face emotion embeddings, face, body and hand landmarks, and gaze and blinking information. Through extensive experiments, we show that our model achieves state-of-the-art results on three key benchmark datasets for depression detection from video by a substantial margin. Our code is publicly available on GitHub.

==> tables/daic-woz-sota.tex <==
% spw=6 | nl=8 nh=4 hd=64 | bs=8 lr=0.0001 | mode (no threshold)
\begin{table}[hbt!]
    \centering
    \caption{Results on the DAIC-WOZ test set. Best results are highlighted in \textbf{bold} and second best results are \underline{underlined}. We show performance across audio-only (A), visual-only (V) and audio-visual (AV) modalities.}
    \begin{adjustbox}{width=0.7\textwidth}
    \begin{tabular}{lcccc}
         \textbf{Method} & \textbf{Modality} & \textbf{F\textsubscript{1}} & \textbf{Precision} & \textbf{Recall} \\ 
         \toprule
         S. Song et al. \cite{song2018daicwoz} & A & 0.46 & 0.32 & \underline{0.86} \\
         Ma et al. \cite{ma2016daicwoz} & A & 0.52 & 0.35 & \textbf{1.00} \\
         J. R. Williamson \cite{williamson2016daicwoz} & A & \underline{0.57} & - & - \\
         P-C. Wei et al. \cite{wei2023daicwoz} & A & \textbf{0.61} & \underline{0.56} & 0.66 \\
         \midrule
         {Perceiver} \cite{jaegle2021perceiver} & A & 0.33{\scriptsize$\pm$0.26} & 0.30{\scriptsize$\pm$0.28} & 0.45{\scriptsize$\pm$0.21} \\
         \textbf{Ours} & A & 0.49{\scriptsize$\pm$0.05} & \textbf{0.58{\scriptsize$\pm$0.05}} & 0.47{\scriptsize$\pm$0.05} \\
         \midrule
         \midrule
         S. Song et al. \cite{song2018daicwoz} & V & 0.50 & 0.60 & 0.43 \\
         J. R. Williamson \cite{williamson2016daicwoz} & V & 0.53 & - & - \\
         P-C. Wei et al. \cite{wei2023daicwoz} & V & 0.61 & 0.64 & 0.58 \\
         \midrule
         {Perceiver} \cite{jaegle2021perceiver} & V & \textbf{0.62{\scriptsize$\pm$0.05}} & \textbf{0.67{\scriptsize$\pm$0.08}} & \textbf{0.62{\scriptsize$\pm$0.05}} \\
         \textbf{Ours} & V & \underline{0.62{\scriptsize$\pm$0.06}} & \underline{0.66{\scriptsize$\pm$0.04}} & \underline{0.61{\scriptsize$\pm$0.06}} \\
         \midrule
         \midrule
         S. Song et al. \cite{song2018daicwoz} & AV & 0.50 & 0.60 & 0.43 \\
         P-C. Wei et al. \cite{wei2023daicwoz} & AV & 0.61 & \textbf{0.78} & 0.50 \\
         \midrule
         {Perceiver} \cite{jaegle2021perceiver} & AV & \underline{0.58{\scriptsize$\pm$0.13}} & \underline{0.75{\scriptsize$\pm$0.05}} & \underline{0.59{\scriptsize$\pm$0.11}} \\
         \textbf{Ours} & AV & \textbf{0.67{\scriptsize$\pm$0.05}} & 0.68{\scriptsize$\pm$0.04} & \textbf{0.66{\scriptsize$\pm$0.06}} \\
    \end{tabular}
    \end{adjustbox}
    \label{tab:daic-woz-sota}
\end{table}

%% F1-WEIGHTED + MODE + VALIDATION THRESHOLDS %%
% M  -> ( precision ) ( recall ) ( f1-score )
% --------------------------------------------------
% A  -> (0.582 ± 0.034) (0.540 ± 0.057) (0.553 ± 0.049)
% V  -> (0.659 ± 0.041) (0.609 ± 0.068) (0.617 ± 0.068)
% AV -> (0.676 ± 0.038) (0.655 ± 0.057) (0.663 ± 0.050)

%% F1-WEIGHTED + MODE + NO THRESHOLDS %%
% M  -> ( precision ) ( recall ) ( f1-score )
% --------------------------------------------------
% A  -> (0.579 ± 0.047) (0.468 ± 0.052) (0.485 ± 0.054)
% V  -> (0.658 ± 0.041) (0.609 ± 0.057) (0.618 ± 0.056)
% AV -> (0.682 ± 0.042) (0.660 ± 0.060) (0.667 ± 0.054)


==> tables/dvlog-modalities.tex <==
\begin{table}[hbt!]
    \centering
    \setlength{\tabcolsep}{4pt}
    \caption{Performance of our method on D-Vlog using different modality combinations, compared to the Perceiver. Best results are highlighted in \textbf{bold} and second best results are \underline{underlined}. Our method is surpassing the strong multi-modal baseline, the Perceiver.}
    \label{tab:dvlog-modalities}
    \begin{adjustbox}{max width=0.7\textwidth}
    \begin{tabular}{lcccc}
        \textbf{Method} & \textbf{Modality} & \textbf{F$_1$} & \textbf{Precision} & \textbf{Recall} \\ 
         \midrule
         \multirow{4}{*}{Perceiver \cite{jaegle2021perceiver}}  & {AV} & 0.69{\scriptsize$\pm$0.06} & 0.72{\scriptsize$\pm$0.07} & 0.69{\scriptsize$\pm$0.13} \\
          & {AV+EYES} & 0.73{\scriptsize$\pm$0.01} & 0.68{\scriptsize$\pm$0.08} & \textbf{0.81{\scriptsize$\pm$0.15}} \\
          & {AV+LM} & 0.67{\scriptsize$\pm$0.13} & 0.70{\scriptsize$\pm$0.14} & 0.74{\scriptsize$\pm$0.28}\\
          & {AV+LM+EYES} & 0.64{\scriptsize$\pm$0.17} & \underline{0.79{\scriptsize$\pm$0.07}} & 0.58{\scriptsize$\pm$0.22}  \\
         \midrule
         % results with spw=9, pt=0.50, mode_presence
         \multirow{4}{*}{\textbf{Ours}} & {AV} & 0.74{\scriptsize$\pm$0.04} & 0.72{\scriptsize$\pm$0.03} & 0.77{\scriptsize$\pm$0.12} \\
          & {AV+EYES} & \underline{0.75{\scriptsize$\pm$0.04}} & 0.72{\scriptsize$\pm$0.03} & \underline{0.79{\scriptsize$\pm$0.12}} \\
          & {AV+LM} & \underline{0.75{\scriptsize$\pm$0.03}} & 0.73{\scriptsize$\pm$0.05} & 0.77{\scriptsize$\pm$ 0.06}\\
          & {AV+LM+EYES} & \textbf{0.78{\scriptsize$\pm$0.01}} & \textbf{0.82{\scriptsize$\pm$0.06}} & 0.74{\scriptsize$\pm$0.05} \\
         % results with spw=6, pt=0.25
         % {Ours} & {AV} & 0.74{\scriptsize$\pm$0.01} & 0.72{\scriptsize$\pm$0.02} & 0.77{\scriptsize$\pm$0.06} \\
         % {Ours} & {AV+EYES} & 0.72{\scriptsize$\pm$0.04} & 0.77{\scriptsize$\pm$0.02} & 0.68{\scriptsize$\pm$0.05} \\
         % {Ours} & {AV+LM} & 0.78{\scriptsize$\pm$0.02} & 0.76{\scriptsize$\pm$0.02} & 0.79{\scriptsize$\pm$0.06} \\
         % {Ours} & {AV+LM+EYES} & 0.72{\scriptsize$\pm$0.04} & 0.73{\scriptsize$\pm$0.01} & 0.71{\scriptsize$\pm$0.07} \\
    \end{tabular}
    \end{adjustbox}
\end{table}

% \begin{table}[hbt!]
%     \centering
%     \setlength{\tabcolsep}{4pt}
%     \caption{{\color{teal}Modality ablation study on D-Vlog test set. Concretely, the different non-verbal behaviour cues described in Section \ref{sec:non-verbal-cues} were considered, where AV, LM, and EYES refer to audio-visual embeddings, landmarks and eye information, respectively.}}
%     \label{tab:dvlog-modalities}
%     \begin{adjustbox}{max width=0.7\textwidth}
%     \begin{tabular}{ccccccccc}
%         \multirow{2}{*}{\textbf{Modality}} &  & \multicolumn{3}{c}{\textbf{Ours}} &  & \multicolumn{3}{c}{\textbf{Perceiver}} \\
%         \cmidrule{3-5} \cmidrule{7-9}
%         &  & F$_1$-Score & Precision & Recall &  & F$_1$-Score & Precision & Recall \\
%         \midrule
%         {AV} &  & 0.77{\scriptsize$\pm$0.01} & 0.70{\scriptsize$\pm$0.04} & 0.85{\scriptsize$\pm$0.07} &  & 0.69{\scriptsize$\pm$0.06} & 0.72{\scriptsize$\pm$0.07} & 0.69{\scriptsize$\pm$0.13} \\
%         {AV+EYES} &  & 0.73{\scriptsize$\pm$0.03} & 0.76{\scriptsize$\pm$0.05} & 0.71{\scriptsize$\pm$0.08} &  & 0.73{\scriptsize$\pm$0.01} & 0.68{\scriptsize$\pm$0.08} & 0.81{\scriptsize$\pm$0.15} \\
%         {AV+LM} &  & 0.75{\scriptsize$\pm$0.03} & 0.73{\scriptsize$\pm$0.05} & 0.77{\scriptsize$\pm$ 0.06} &  & 0.67{\scriptsize$\pm$0.13} & 0.70{\scriptsize$\pm$0.14} & 0.74{\scriptsize$\pm$0.28} \\
%         {AV+LM+EYES} &  & 0.78{\scriptsize$\pm$0.01} & 0.82{\scriptsize$\pm$0.06} & 0.74{\scriptsize$\pm$0.05} &  & 0.64{\scriptsize$\pm$0.17} & 0.79{\scriptsize$\pm$0.07} & 0.58{\scriptsize$\pm$0.22} \\
%     \end{tabular}
%     \end{adjustbox}
% \end{table}

==> tables/dvlog-sota.tex <==
% spw=9 | nl=8 nh=8 hd=32 | bs=8 lr=0.001 | mode + no threshold?
\begin{table}[hbt!]
    \centering
    % \setlength{\tabcolsep}{8pt}
    \caption{Results on the D-Vlog test set compared to existing approaches. Best results are highlighted in \textbf{bold} and second best results are \underline{underlined}.}
    \label{tab:dvlog-sota}
    \begin{adjustbox}{width=0.7\textwidth}
    \begin{tabular}{lp{1.5cm}p{1.5cm}ccc}
         \textbf{Method} & \textbf{Original Split} & \textbf{Additional Modalities} & \textbf{F$_1$} & \textbf{Precision} & \textbf{Recall} \\ 
         \toprule
         {Yoon et al.} \cite{yoon2022dvlog} & \checkmark & \xmark & 0.64 & 0.65 & 0.66 \\
         {Nguyen et al.} \cite{nguyenmultimodal} & \checkmark & \xmark & 0.64 & 0.66 & 0.64 \\
         {Zheng et al.} \cite{zheng2023two} & \checkmark & \xmark & 0.65 & 0.65 & 0.65 \\
         {Zhou et al.} \cite{zhou2022tamfn} & \checkmark & \xmark & 0.66 & 0.66 & 0.67 \\
         {Zhou et al.} \cite{zhou2023caiinet} & \checkmark & \xmark & 0.67 & 0.67 & 0.67 \\ 
         {Tao et al.} \cite{tao2023depressive} & \checkmark & \xmark & \underline{0.75} & \textbf{0.73} & 0.78 \\ 
         \midrule
         {Perceiver} \cite{jaegle2021perceiver} & \checkmark & \xmark & 0.74{\scriptsize$\pm$0.01} & 0.67{\scriptsize$\pm$0.03} & \underline{0.84{\scriptsize$\pm$0.07}} \\
         {\textbf{Ours}} & \checkmark & \xmark & \textbf{0.76{\scriptsize$\pm$0.01}} & \underline{0.67{\scriptsize$\pm$0.01}} & \textbf{0.85{\scriptsize$\pm$0.01}} \\
         \midrule
         \midrule
         {Perceiver} \cite{jaegle2021perceiver} & \xmark & \xmark & 0.72{\scriptsize$\pm$0.01} & \underline{0.66{\scriptsize$\pm$0.03}} & 0.80{\scriptsize$\pm$0.03} \\
         {Perceiver} \cite{jaegle2021perceiver} & \xmark & \checkmark & 0.73{\scriptsize$\pm$0.01} & 0.66{\scriptsize$\pm$0.09} & \underline{0.84{\scriptsize$\pm$0.14}} \\
         {\textbf{Ours}} & \xmark & \xmark & \underline{0.73{\scriptsize$\pm$0.01}} & 0.62{\scriptsize$\pm$0.01} & \textbf{0.89{\scriptsize$\pm$0.05}} \\
         {\textbf{Ours}} & \xmark & \checkmark & \textbf{0.78{\scriptsize$\pm$0.01}} & \textbf{0.82{\scriptsize$\pm$0.06}} & 0.74{\scriptsize$\pm$0.05} \\
    \end{tabular}
    \end{adjustbox}
\end{table}




==> tables/e-daic-sota.tex <==
% spw=6 | nl=8 nh=4 hd=64 | bs=8 lr=0.0001 | mode (no threshold)
\begin{table}[hbt!]
    \centering
    \caption{Results on the E-DAIC test set. Best results are highlighted in \textbf{bold} and second best results are \underline{underlined}. We show performance across audio-only (A), visual-only (V) and audio-visual (AV) modalities.}
    \label{tab:e-daic-sota}
    \begin{adjustbox}{width=0.6\textwidth}
    \begin{tabular}{lcccc}
        \textbf{Method} & \textbf{Modality} & \textbf{F$_1$} & \textbf{Precision} & \textbf{Recall} \\
         \midrule
         \multirow{3}{*}{Perceiver \cite{jaegle2021perceiver}}  & A & 0.36{\scriptsize$\pm$0.17} & \underline{0.66{\scriptsize$\pm$0.12}} & 0.41{\scriptsize$\pm$0.09} \\
          & V & 0.39{\scriptsize$\pm$0.22} & 0.50{\scriptsize$\pm$0.26} & 0.48{\scriptsize$\pm$0.18} \\
         & AV & \underline{0.53{\scriptsize$\pm$0.09}} & 0.54{\scriptsize$\pm$0.05} & \underline{0.54{\scriptsize$\pm$0.11}} \\
         \midrule
         \multirow{3}{*}{\textbf{Ours}} & A & 0.51{\scriptsize$\pm$0.11} & \textbf{0.71{\scriptsize$\pm$0.05}} & 0.52{\scriptsize$\pm$0.08} \\
          & V & 0.50{\scriptsize$\pm$0.08} & 0.58{\scriptsize$\pm$0.05} & 0.49{\scriptsize$\pm$0.07} \\
         & AV & \textbf{0.56{\scriptsize$\pm$0.12}} & 0.59{\scriptsize$\pm$0.07} &\textbf{ 0.58{\scriptsize$\pm$0.13}} \\
    \end{tabular}
    \end{adjustbox}
\end{table}

% \begin{table}[hbt!]
%     \centering
%     \setlength{\tabcolsep}{4pt}
%     \caption{{\color{teal}Results on the E-DAIC test set. The best results are highlighted in \textbf{bold}. A, V and AV refer to those experiments that used audio-, video-, or audiovisual-based features, respectively. It should be noted that current state of the art explore semantic-based features extracted from the transcript, achieving performances around 0.950 F\textsubscript{1}-Score \cite{zheng2023two}. However, to the best of our knowledge, our experiments are the first ones addressing the task of binary depression detection from a non-verbal perspective.}}
%     \label{tab:e-daic-sota}
%     \begin{tabular}{ccccccccc}
%         \multirow{2}{*}{\textbf{Modality}} &  & \multicolumn{3}{c}{\textbf{Ours}} &  & \multicolumn{3}{c}{\textbf{Perceiver}} \\
%         \cmidrule{3-5} \cmidrule{7-9}
%         &  & F$_1$-Score & Precision & Recall &  & F$_1$-Score & Precision & Recall \\
%         \midrule
%         A &  & 0.63{\scriptsize$\pm$0.06} & 0.70{\scriptsize$\pm$0.04} & 0.61{\scriptsize$\pm$0.06} &  & 0.52{\scriptsize$\pm$0.10} & 0.59{\scriptsize$\pm$0.13} & 0.57{\scriptsize$\pm$0.10} \\
%         V &  & 0.58{\scriptsize$\pm$0.08} & 0.60{\scriptsize$\pm$0.07} & 0.60{\scriptsize$\pm$0.12} &  & 0.32{\scriptsize$\pm$0.22} & 0.36{\scriptsize$\pm$0.25} & 0.42{\scriptsize$\pm$0.17} \\
%         AV &  & 0.56{\scriptsize$\pm$0.04} & 0.58{\scriptsize$\pm$0.07} & 0.59{\scriptsize$\pm$0.06} &  & 0.47{\scriptsize$\pm$0.17} & 0.50{\scriptsize$\pm$0.11} & 0.52{\scriptsize$\pm$0.15} \\
%     \end{tabular}
% \end{table}

%%%%%%%%%%%%%%%%%%%%
%% BASELINE MODEL %%
%%%%%%%%%%%%%%%%%%%%
%% F1-WEIGHTED + MODE + VALIDATION THRESHOLDS %%
% M  -> ( precision ) ( recall ) ( f1-score )
% --------------------------------------------------
% A  -> (0.687 ± 0.153) (0.700 ± 0.023) (0.597 ± 0.020)
% V  -> (0.690 ± 0.070) (0.707 ± 0.020) (0.641 ± 0.027)
% AV -> (0.545 ± 0.089) (0.682 ± 0.015) (0.576 ± 0.023)

%% F1-WEIGHTED + MODE + NO THRESHOLDS %%
% M  -> ( precision ) ( recall ) ( f1-score )
% --------------------------------------------------
% A  -> (0.702 ± 0.037) (0.614 ± 0.060) (0.625 ± 0.058)
% V  -> (0.603 ± 0.065) (0.604 ± 0.115) (0.584 ± 0.082)
% AV -> (0.580 ± 0.074) (0.586 ± 0.060) (0.561 ± 0.042)


